BCNN: Binary Complex Neural Network

Binarized neural networks, or BNNs, show great promise in edge-side applications with resource limited hardware, but raise the concerns of reduced accuracy. Motivated by the complex neural networks, in this paper we introduce complex representation into the BNNs and propose Binary complex neural network -- a novel network design that processes binary complex inputs and weights through complex convolution, but still can harvest the extraordinary computation efficiency of BNNs. To ensure fast convergence rate, we propose novel BCNN based batch normalization function and weight initialization function. Experimental results on Cifar10 and ImageNet using state-of-the-art network models (e.g., ResNet, ResNetE and NIN) show that BCNN can achieve better accuracy compared to the original BNN models. BCNN improves BNN by strengthening its learning capability through complex representation and extending its applicability to complex-valued input data. The source code of BCNN will be released on GitHub.

==> backup.tex <==





 
% In the forward pass of BNN, the combination of BN layer and activation sign binarization can be convert to a thresholding. Without loss of generality, assuming $\gamma$ is positive.
% \[ sign(h) =  \left \{ \begin{array}{ccc}
% +1 \qquad  z\geq \tau \\
% -1 \qquad z< \tau \end{array} \right   \qquad \tau = \frac{-\beta\sqrt{\sigma^2}+\epsilon}{\gamma}+\mu 
% \] 

% This conversion is very useful for digital design since thresholding is much efficiently than arithmetic that required in BN layer.



\iffalse
\[ V =  \left( \begin{array}{ccc}
V_{rr} & V_{ri}\\
V_{ir} & V_{ii} \end{array}\right) = 
\left( \begin{array}{ccc}
Cov(R\{z\},R\{z\}) & Cov(R\{z\},I\{z\})\\
Cov(I\{z\},R\{z\}) & Cov(I\{z\},I\{z\}) \end{array}\right)
\]
\[ \gamma =  \left( \begin{array}{ccc}
\gamma_{rr} & \gamma_{ri}\\
\gamma_{ri} & \gamma_{ii} \end{array}\right)
\]
\fi

% we came up with a new batch normalization for complex binary network, which has less computation.

% As we can see, during the complex batch normalization computing, the real part and imaginary part are related to each other, there is no way to convert into thresholding, which is useful for BNN Accelerated implementation. To address this problem, A new simple and efficient complex batch normalization is proposed for BCNN. 
